Boosting the Performance of Object Tracking with a Half-Precision Particle Filter on GPU

High-performance GPU-accelerated particle filter methods are critical for object detection applications, ranging from autonomous driving, robot localization, to time-series prediction. In this work, we investigate the design, development and optimization of particle-filter using half-precision on CUDA cores and compare their performance and accuracy with single- and double-precision baselines on Nvidia V100, A100, A40 and T4 GPUs. To mitigate numerical instability and precision losses, we introduce algorithmic changes in the particle filters. Using half-precision leads to a performance improvement of 1.5-2x and 2.5-4.6x with respect to single- and double-precision baselines respectively, at the cost of a relatively small loss of accuracy.

==> old/table_timing.tex <==
\begin{table*}[]
    \centering
    \caption{Average running time for likelihood, weighting, normalizing, and resampling kernels on three different precision over 100 iterations of the particle filter. The experiment was performed two times using 1,024 and 2,048 numbers of particles. The input size was fixed as a 100-frame video of size $256 \times 256$. The running time was captured by using nvprof. }
    \label{tab:runtime}
    \begin{tabular}{lcccccccccccc}
        \toprule &
        \multicolumn{8}{c}{Average Running Time in $\mu$s} \\
        \cmidrule{2-9} Kernel &
        \multicolumn{2}{c}{Likelihood} & \multicolumn{2}{c}{Weighting} & 
        \multicolumn{2}{c}{Normalizing} & \multicolumn{2}{c}{Resampling} \\
        \cmidrule(lr){2-3} 
        \cmidrule(lr){4-5} 
        \cmidrule(lr){6-7} 
        \cmidrule(lr){8-9} 
        Nb. of Particles 
        & 1024 & 2048 
        & 1024 & 2048 
        & 1024 & 2048 
        & 1024 & 2048 \\
        \midrule 
        FP64 & 69.91 & 135.10 & 12.01 & 12.00 & 111.98 & 241.62 & 259.71 & 566.97 \\
        FP32 & 24.47 & 39.19 & \textbf{4.47} & \textbf{4.56} & 54.53 & 117.23 & 112.24 & 227.42 \\
        FP16 & \textbf{19.05} & \textbf{27.77} & 5.03 & 5.37 & \textbf{30.37} & \textbf{68.03} & \textbf{73.83} & \textbf{165.44} \\
        \midrule 
        FP32 Speedup & 2.86x & 3.45x & \textbf{2.68x} & \textbf{2.63x} & 2.05x & 2.06x & 2.31x & 2.49x \\
        FP16 Speedup & \textbf{3.67x} & \textbf{4.87x} & 2.39x & 2.23x & \textbf{3.69x} & \textbf{3.55x} & \textbf{3.52x} & \textbf{3.43x} \\
        \bottomrule
    \end{tabular}
\end{table*}
